XPASC: Measuring Generalization in Weak Supervision by Explainability and Association

Weak supervision is leveraged in a wide range of domains and tasks due to its ability to create massive amounts of labeled data, requiring only little manual effort. Standard approaches use labeling functions to specify signals that are relevant for the labeling. It has been conjectured that weakly supervised models over-rely on those signals and as a result suffer from overfitting. To verify this assumption, we introduce a novel method, XPASC (eXPlainability-Association SCore), for measuring the generalization of a model trained with a weakly supervised dataset. Considering the occurrences of features, classes and labeling functions in a dataset, XPASC takes into account the relevance of each feature for the predictions of the model as well as the associations of the feature with the class and the labeling function, respectively. The association in XPASC can be measured in two variants: XPASC-CHI SQAURE measures associations relative to their statistical significance, while XPASC-PPMI measures association strength more generally. We use XPASC to analyze KnowMAN, an adversarial architecture intended to control the degree of generalization from the labeling functions and thus to mitigate the problem of overfitting. On one hand, we show that KnowMAN is able to control the degree of generalization through a hyperparameter. On the other hand, results and qualitative analysis show that generalization and performance do not relate one-to-one, and that the highest degree of generalization does not necessarily imply the best performance. Therefore methods that allow for controlling the amount of generalization can achieve the right degree of benign overfitting. Our contributions in this study are i) the XPASC score to measure generalization in weakly-supervised models, ii) evaluation of XPASC across datasets and models and iii) the release of the XPASC implementation.

==> ReviewerComments.tex <==
Reviewer(s)' Comments to Author:

Reviewer: 1

Comments to the Author
Excellent work! I have two comments on the experiments:
1. All the included datasets are binary classification- authors may want to include datasets that are multiclass classification and find this project useful (https://github.com/JieyuZ2/wrench) since it contains a collection of datasets for weak supervision.
2. Authors compared KNOWMAN against MV and Snorkel, but the latter two are label models that do not input data features. Thus, authors may want to include other weak supervision methods that also input data features as KNOWMAN, for example, the WeaSEL model (https://openreview.net/forum?id=gbcsmD3Iznu) .

Related work that authors may want to include in the discussion:
1.Understanding Programmatic Weak Supervision via Source-aware Influence Function (https://arxiv.org/abs/2205.12879)
2.A Survey on Programmatic Weak Supervision.  Introduction (https://arxiv.org/abs/2202.05433)

Minor comments:
Several references are in arxiv version, but they were already published in conferences. The authors may want to double-check their references to ensure all published paper are appropriately cited.


#################### Answer ####################
Dear reviewer, thank you for your valuable feedback. 
We have the following comments regarding your points: 
1.	We added a multi-class dataset from the WRENCH benchmark, TREC. Please find the new content and experiments regarding that dataset in the paper.
2.	We included WeaSEL as a model in our experimentation, please find the new contents in the paper. For the SPOUSE dataset WeaSEL gives a result of 0\% F1 score. This is also reported in Stephan et al. (Stephan, A., Kougia, V., & Roth, B. (2022). SepLL: Separating Latent Class Labels from Weak Supervision Noise. ArXiv, abs/2210.13898.) and in addition we had email conversation with the author of WeaSEL w.r.t. the issue. 
At the moment the issue is unsolved on their side, since their original paper does not use pre-trained language models, as we do apply them.
3.	Thank you for the suggestion of this interesting related work. We included them in the paper (see Introduction and Related Work)
4.	We double-checked and adjusted our references carefully.
#################################################


Reviewer: 2

Comments to the Author
This paper proposes a metric, called eXPlainability-Association SCore (XPASC) to measure the degree of generalization of weakly supervised models.  The paper claims a high XPASC is expected to indicate a greater generalization from weak sources.  XPASC combines two factors: (1) the importance of a feature for the classification of an instance, called the explainability score, and (2) the correlation of a feature with a class and a labeling function, called the association score.  The paper evaluates XPASC using three datasets and three weakly supervised models.

Strengths:
1) The paper conducts extensive experiments and analyses with numerous examples.
2) The paper verifies expected behaviors of XPASC by controlling a hyperparameter of the KnowMAN model.
3) The paper is well organized and easy to follow its contents.

Weaknesses:
1) My major concern is that the paper ignores the notion of underfitting, thereby making the notion of generalization misleading.  I think what XPASC attempts to measure is the degree of underfitting to labeling functions, not the degree of generalization.  In Figure 5, for example, I suspect Snorkel-DP is actually underfitting, and KnowMAN could have higher generalization performance on out-domain data.  The same suspicion goes to the case of lambda = 4 in Figure 6 for which the paper did not explain why the case of lambda = 4 produces a worse performance than the case of lambda = 2.  In another word, due to the ignorance of underfitting, XPASC is not informative enough to rule out the two extremes of overfitting and underfitting to identify the actual sweet spot of high generalization.

2) The association score seems to be the core of XPASC because a larger score means less reliance on labeling functions.  However, it is not clear how important the explainability score is for XPASC.  The formalization of XPASC would be more convincing if it clarified the role of the explainability score and provided an ablation study to analyze its effect.

3) The paper defines features as single tokens of an input sentence.  While this formalization of features may allow for systematic analysis, they are rather limited features, not reflecting realistic labeling functions.  For example, sentiment analysis may want to consider a little more complicated features such as token pairs, e.g., (not, good).  Transformer-based models such as DistilBERT used in the paper are likely to leverage such complicated features through their self-attention mechanism.  The paper would be more insightful if it showed how XPASC behaves when using more useful features for predictions or more faithful features that are likely to be employed by target models.

Below are some minor comments about stylistic issues, etc.
- Section 1 (Page 3): valuesof -> values of
- Section 3 (Page 5): The sentence "To calculate explainability, ..." is ungrammatical.
- Section 5.2.1: a slightly higher XPASC then the KNOWMAL models -> a slightly higher XPASC *than* the KNOWMAL models

#################### Answer ####################
Dear reviewer, thank you for your positive feedback as well as the critical remarks.
We would like to address all the issues as follows:
1) XPASC aims to measure generalization from the weak signals/ labeling functions. 
Measuring the fit to the labeling functions only, would capture overfitting only.
However, we measure the fit to the labeling functions (association contained in matrix L) in contrast to the fit to the class (association contained in matrix C) with Formula 3. 
By doing so, we argue that underfitting to the labeling functions (which is the same as less overfitting to them) at the same time increases generalization to the class. 
---
The parameter lambda is meant to control the degree of discarding the labeling function information. 
Though, the information contained in the labeling functions may be valuable. 
Discarding the information too much will harm the system’s performance and by tuning lambda we can find the sweet spot, where the information is discarded only to an extent that helps with better model prediction. 
That is the reason why, in the cases you mentioned, the performance is decreasing. 

2)	The influence of explainability and association on XPASC are equal. We reworked the relevant passages to make that point clearer. 
As you can see from the XPASC formula (number 11 in the paper), both components are multiplied without weighting and therefore also contribute in equal parts.
If one of the components is left out the score will be meaningless. Explainability and association are always distributed over features, but the interesting part is their interaction.
3)	We like the idea to consider other features for XPASC. 
Note however, that labeling functions can already span multiple tokens (it would be still counted as one match).
To calculate the association we need some features that have a countable surface form, because the formulation of PPMI takes the total occurrences vs. expected occurrences into account. 
Using attention weights as features would not allow to do so. 
In addition our approach covers the issue of token pairs already in the sense that the explainability by occlusion will change for both tokens of a token pair, indicating that both tokens are relevant for prediction.
Therefore we think that the surface forms (tokens) as features are well suited for XPASC and carry a very high level of information.
4)	We addressed the stylistic issues you mentioned and did check the paper again for misspellings and ungrammaticality.
#################################################

 

Reviewer: 3

Comments to the Author
This paper proposes a new metric XPASC to measure the generalization of weakly-supervised models by labeling functions. 

Advantages:
1. The motivation and the proposed method may be interesting to the community. I think the generalization of models trained by weak supervision from labeling functions is important to measure if models just fit these labeling functions or learn information related to the classification types.

2. Few studies working on the problem, so I think the novelty and originality are good enough.

3. Although writing needs to be improved, the paper is easy to understand and readers follow the intuition behind the idea.

4. The results from different datasets and models make sense and the authors provide a detailed analysis of them.

Negativeness:
1. The value of this score is too small which is hard to compare. Better to find a way to normalize them from 0 to 1.

2. Better to compare more weakly supervised methods.

3. Writing needs to be improved. Have some typos, e.g., "valuesof" in the first paragraph of page 3.

One question: Why are all XPASC scores in Figures 3,4,5 close to 1 but in Figures 6,7 they are negative?

#################### Answer ####################
Dear reviewer, thank you for the remarks and the feedback. We would like to answer all of the points as follows: 
1)	We included a dedicated section about the normalization of the score and the behaviour of XPASC w.r.t. to normalization. Please find the details in section 5.2.3 Magnitude of XPASC now.
The different numbers had been due to the fact that we normalized the values to be positive (we subtracted the negative XPASC from 1) for Figures 3,4,5 in order to make the bar plots easier to display. We now adjusted the formula to give positive results and all figures are consistent w.r.t. that issue now.
2)	We included WeaSEL, another model for weak supervision, to our experiments. Please find the new contents in the paper.  For the SPOUSE dataset WeaSEL gives a result of 0\% F1 score. This is also reported in Stephan et al. (Stephan, A., Kougia, V., & Roth, B. (2022). SepLL: Separating Latent Class Labels from Weak Supervision Noise. ArXiv, abs/2210.13898.) and in addition we had email conversation with the author of WeaSEL w.r.t.the issue. At the moment the issue is unsolved on their side, since their original paper does not use pre-trained language models, as we do apply them.
3)	We checked our paper again for misspellings, ungrammaticality and stylistic issues to improve the writing. 
#################################################


